Maliva: Using Machine Learning to Rewrite Visualization Queries Under Time Constraints

We consider data-visualization systems where a middleware layer translates a frontend request to a SQL query to a backend database to compute visual results. We study the problem of answering a visualization request within a limited time constraint due to the responsiveness requirement. We explore the optimization options of rewriting an original query by adding hints and/or doing approximations so that the total time is within the time constraint. We develop a novel middleware solution called Maliva based on machine learning (ML) techniques. It applies the Markov Decision Process (MDP) model to decide how to rewrite queries and uses training instances to learn an agent to make a sequence of decisions judiciously for an online request. We give a full specification of the technique, including how to construct an MDP model, how to train an agent, and how to use approximating rewrite options. Our experiments on both real and synthetic datasets show that Maliva performs significantly better than a baseline solution that does not do any rewriting, in terms of both the probability of serving requests interactively and query execution time.

==> overflow.tex <==
%%%%%
% Previous Section 4.1 Markov Decision Process (MDP)
%%%%%
\subsection{Markov Decision Process (MDP)\label{subsec:mdp-preliminaries}}

\begin{figure}[htb]
  \centering
  \includegraphics[width=0.9\linewidth]{figures/mdp}
  \caption{The agent-environment interaction in a Markov decision process.}
  \label{fig:agent-environment}
\end{figure}

\boldstart{MDP}~\cite{books/lib/SuttonB98} is a formalization of sequential decision-making problems where an agent learns to achieve a goal from interaction with an environment. Formally, an MDP is a 5-tuple $(S, A, \mathcal{T}, \mathcal{R}, \gamma)$~\cite{conf/sigmod/SikdarJ20}. As shown in Figure~\ref{fig:agent-environment}, at time step $t$, the agent receives a representation of the environment's \emph{state}, $s_t \in S$, and on that basis selects an \emph{action}, $a_t \in A$, or alternatively from $A_{s_t}$, the set of actions available from state $s_t$.  At time step $t+1$, in part as a consequence of its action, the agent receives a numerical \emph{reward}, $r_{t+1} \in \mathbb{R}$, and finds itself in a new state, $s_{t+1}$. The probability $P_{a_t}(s_t, s_{t+1})$ the agent transits to state $s_{t+1}$ from state $s_t$ taking action $a_t$ is defined by a \emph{transition function} $\mathcal{T}$. The received reward $R_{a_t}(s_t, s_{t+1})$ is defined by a \emph{reward function} $\mathcal{R}$. If $P_{a_t}(s_t, s_{t+1})$ is conditionally independent from previous states and actions, it is said to satisfy the \emph{Markov property}. The discount factor $\gamma \in [0,1]$ balances the importance of future rewards compared to immediate rewards. The interactions happen continually, and the agent seeks to maximize the cumulative reward over time through its choice of actions.



A solution to an MDP problem is a \emph{policy} $\pi$ that specifies the action $\pi(s)$ chosen by the agent at state $s$. The goal is to find a good policy that maximizes the total reward the agent will receive. From the start state $s_0$, the expected total reward for policy $\pi$ is defined as 

$$
V^{\pi}(s_0) = E\left[\sum_{t=0}^{\infty} \gamma^t R_{a_t}(s_t, s_{t+1}) \mid \pi\right].
$$

To solve an MDP problem, we want to find a policy $\pi^*$ that maximizes the expected total reward:

$$
\pi^* = argmax_{\pi} V^{\pi}(s_0).
$$







%%%%%
% Previous Section 6 Hybrid Approach to Reduce Response Time
%%%%%

\section{Hybrid Approach to Reduce Response Time\label{sec:hybrid-approach}}

As we will see in Section~\ref{sec:experiments}, \sysName can use hints to help the database generate a viable execution plan.  On the other hand, for ``easy'' queries (those with many viable plans), in some cases the plan generated by the MDP technique may run slower than the one given by the database optimizer. %For queries with few viable plans (e.g., only one), the MDP-based approach can plan smartly by learning extra information from exploring different plans and outperform the database optimizer by generating a viable plan with a much higher chance.  For queries with many viable plans, the database optimizer outperforms the MDP-based approach due to the extra planning time needed by the MDP-based approach. In this section, we study the problem of how to reduce the average query response time using an ML-based hybrid solution.
This is mainly due to the computational overhead introduced by the MDP-based method.  Next we discuss how to further reduce the average query response time using an ML-based hybrid solution.

\boldstart{Query classifier.} We introduce a new component called {\em Query Classifier} to the query generator module in \sysName, as shown in Figure~\ref{fig:query-classifier}. This component extracts features from an incoming visualization request, and decides whether to use the MDP agent to generate a hinted query or forward the original query directly to the database. The goal is to minimize the query execution time.

\begin{figure}[ht]
  \centering
  \includegraphics[width=0.8\linewidth]{figures/query-classifier}
  \caption{Hybrid solution that uses a query classifier to choose one of the two approaches. }
  \label{fig:query-classifier}
\end{figure}

\boldstart{Extracting features.}  For a visualization request, we use estimated selectivity values of its filtering conditions as features of the classifier. A critical requirement is that this feature-extraction process should be fast. Many solutions are available.  For instance, for numerical range conditions, we can use histogram-based methods (e.g.,~\cite{conf/sigmod/PoosalaIHS96, conf/sigmod/MatiasVW98, conf/pods/GuhaKS02,books/daglib/0011128}).  To estimate selectivity of keyword conditions, we can adopt existing techniques, including those for conjunctive conditions~\cite{journals/jcss/ChenKKM03, conf/edbt/YuKZ06}.

%{\em Textual conditions.} To estimate the selectivity of a keyword (e.g., {\tt covid}), we build a hash map with words as the keys and their selectivity as the value. For a condition with a single keyword, we look up the hash table to get its selectivity.  For textual selections with multiple keywords, we estimate the selectivity value for the conjunctive condition using existing techniques~\cite{journals/jcss/ChenKKM03, conf/edbt/YuKZ06}.

%{\em Categorical conditions.} For this type of conditions, we build a hash map with all possible categorical values as the keys and the selectivity of each category as the values, which can be obtained by running a aggregation query on the table. For a new query, we look up the hash map and compute the selectivity for the categorical selection condition.



% For example, we could adopt the method from~\cite{books/daglib/0011128} and extend it to a hierarchy. We briefly explain the main idea of a hierarchy of equi-width histograms with different bucket widths in our setting.  Consider a temporal selection condition on the \texttt{created\_at} attribute. We build a hierarchy of histograms of days, weeks, and months, as shown in Figure~\ref{fig:numerical-condition-feature}. To estimate the selectivity of a range predicate [11/1/2020, 12/2/2020], we use the monthly histogram to compute the selectivity for November, and use the daily histogram to compute the selectivity of the remaining sub-range from 12/1/2020 to 12/2/2020. The summation of the two values will be an estimated selectivity of the range condition.

% \begin{figure}[ht]
%   \centering
%   \includegraphics[width=0.9\linewidth]{figures/numerical-condition-feature}
%   \caption{An example of using hierarchical histograms to estimate the selectivity of a numerical range condition.}
%   \label{fig:numerical-condition-feature}
% \end{figure}



%% Remove as it's irrelevant

%% In reality, building the histograms and hash maps on the base table can be expensive if the base table has too many records. We can first obtain a random sample from the base table and then build the histograms and hash maps on the sample. For example, we used a 1\% sample to build the histograms and hash maps in all our experiments.


%\boldstart{Offline Training and Online Classification.}  

We train a query classifier offline using a set of training queries using their extracted query features. For each query, we compare the response times of the baseline that relies on the database optimizer and the MDP-based approaches. We then label the query with the approach that has a lower response time. With all training queries labeled, we apply a supervised learning method (e.g., KNN) to train the query classifier. At run time, we use the trained model to classify new queries online. Based on the prediction of the query classifier, we can either use the MDP agent to add hints, or send the query directly to the database.
